Left-Deep Join Order Selection with Higher-Order Unconstrained Binary Optimization on Quantum Computers

Join order optimization is among the most crucial query optimization problems, and its central position is also evident in the new research field where quantum computing is applied to database optimization and data management. In the field, join order optimization is the most studied database problem, usually tackled with a quadratic unconstrained binary optimization model, which is solved with various meta-heuristics such as quantum annealing, quantum approximate optimization algorithm, or variational quantum eigensolver. In this work, we continue developing quantum computing techniques for join order optimization by presenting three novel quantum optimization algorithms. These algorithms are based on a higher-order unconstrained binary optimization model, which is a generalization of the quadratic model and has not previously been applied to database problems. Theoretically, these optimization problems naturally map to universal quantum computers and quantum annealers. Compared to previous research, two of our algorithms are the first quantum algorithms to precisely model the join order cost function. We prove theoretical bounds by showing that these two methods encode the same plans as the dynamic programming algorithm without cross-products, which provides the optimal result up to cross-products. The third algorithm reaches at least as good plans as the greedy algorithm without cross-products. These results set an important theoretical connection between the classical and quantum algorithms for join order selection, which has not been studied in the previous research. To demonstrate our algorithms' practical usability, we have conducted an experimental evaluation on thousands of clique, cycle, star, tree, and chain query graphs using quantum and classical solvers.

==> sections/greedy_bushy_trees.tex <==
\section{Greedy, weighted, maximal matching -based method for bushy tree selection}

==> sections/old_constraints.tex <==
\subsection{Select exactly $|V| - 1$ many different edges from query graph.}
Every edge corresponding to a join in a query graph should appear in the solution either 0 or 1 times. To encode this constraint, for each join, we introduce an auxiliary variable that counts whether the join appears in the solution. This adds $|E|$ new variables to the model. We denote these auxiliary variables as $x_{ij}$ for each $(R_i, R_j) \in E$.

We utilize a similar structure as in Eq.~\eqref{eq:hubo_combinations}, but instead of fixing the number of selected variables to be exactly one, we select either 1 or 0 variables to be true. The constraint that encodes this is the following objective:
\begin{equation}\label{eq:exactly_v1_different_joins}
    H_2 = \sum_{(R_i, R_j) \in E}\left( x_{ij} - \sum_{r = 0}^{|V| - 2}x_{i,j}^{r} \right)^2.
\end{equation}
If the auxiliary variable $x_{ij} = 1$, then the objective function is minimized when precisely one variable of type $x_{i,j}^{r}$ is selected true.

Then, we must select exactly $|V| - 1$ many auxiliary variables to be true. The following constraint achieves this:
\begin{equation}
    H_{\text{aux}} = \left( |V| - 1 - \sum_{(R_i, R_j) \in E}x_{ij} \right)^2.
\end{equation}

\subsection{Ranks should be arranged so the selected joins produce a left-deep tree.}
We use the variables to explain the idea behind this constraint. Variable $x_{k,l}^{r+1}$ with rank $r + 1$ should have the following relationship with the variable $x_{i,j}^{r}$ with rank $r$: if $R_i \neq R_k$ and $R_j \neq R_l$ in the query graph, then the product $x_{i,j}^{r}x_{k,l}^{r+1}$ should have a positive coefficient, i.e., these variable combinations are penalized. In other words, we always want consecutive joins to share a common table. This constraint necessarily encodes the fact that the plan is left-deep. The objective function for this is the following:
\begin{equation}\label{eq:connected_ranks}
    H_3 = A\sum_{r = 0}^{|V| - 3}x_{i,j}^{r}x_{k,l}^{r+1},
\end{equation}
for all $R_i \neq R_k$ and $R_j \neq R_l$ and where $A$ is the positive penalizing term.

\subsection{Every table has to be joined.}
This constraint is again similar to constraints \eqref{eq:hubo_combinations} and \eqref{eq:exactly_v1_different_joins} where we wanted to select a specific number of variables to be true. In this case, we want to force a constraint that guarantees that every table appears at least once in the solution returned by the binary model. We proceed with the trick developed in \cite{lucas}, where we can encode an integer value using binary variables.
\begin{equation}\label{eq:every_table_joined_once}
    H_4 = \sum_{R_i \in V} \left( x_{i} - \sum_{(R_i, R_j) \in E} x_{i,j}^{r} \right)^2,
\end{equation}
where $x_i = \sum_{n = 0}^{M - 1}2^n y^{i}_{n} + (N + 1 - M)y_{M}^{i}$ where $M = \lfloor \log(|V| - 1) \rfloor$ and $y_{k}^{i}$ are auxiliary variables for each $i = 0, \ldots, |V| - 1$ and $k = 0, \ldots, M$. Again, we get two different HUBO formulations with these validity constraints and the previous two cost functions.

==> sections/thoughts.tex <==
The join order selection problem is dynamic in the sense that we perform one or multiple joins at each step until we reach the final result. Joins that we perform earlier affect the total cost in the end. This dynamic time element makes encoding the problem with binary models challenging since there is no natural way of doing this encoding. Most of the previously modeled optimization problems are static compared to join order selection \cite{lucas}.

HUBO problems are hard to solve classically. Constructing problems that admit natural HUBO formulation would ideally produce use cases that could be solved more efficiently with quantum devices than classical devices. So far, at least in this problem instance, we have not experienced this advantage. Considering how the number of HUBO variables (which is a one-to-one correspondence with a required number of qubits) is mapped to the equivalent QUBO formulation, we see how HUBO problems are clearly more expressible.

==> sections/universal.tex <==
\subsubsection{Universal quantum computers}

The reduction methods are especially meant for quantum annealers. Universal quantum computers are able to encode HUBO problems without the reduction~\cite{10313783, 10.1145/3478519}. This is an interesting practical difference between universal quantum computing and quantum annealing.

Since previous research has not explicitly formulated HUBOs for universal quantum computers, we develop, describe, and apply the method in this paper. We implement a similar approach as QAOA with a modified parametrization. First, we translate the HUBO problem into the equivalent Ising Hamiltonian
\begin{equation}\label{eq:hubo_to_hamiltonian}
    \sum_{S \subset [n]}\alpha_{S}\prod_{i \in S}x_i \mapsto \sum_{S \subset [n]}\alpha_{S}\prod_{i \in S}\frac{I - \sigma_{z}^{i}}{2},
\end{equation}
where $I$ is the identity matrix and $\sigma_{z}^{i}$ is the matrix for the Pauli-Z gate acting on qubit $i$. Based on quantum mechanics, the minimum eigenstate and the corresponding minimum eigenvector of Hamiltonian $H$ solve the HUBO optimization problem. 

Next, we utilized a modified QAOA routine to find the minimum eigenvalue and eigenstate with a universal quantum computer. The original QAOA \cite{farhi2014quantum} has been widely applied to solve QUBOs, but the same algorithm can be used to find the minimum eigenvalue and eigenstate of Hamiltonians corresponding HUBOs. The key ingredients of the algorithm are two parametrized unitaries called cost and mixer. These unitaries are layered $p$ times. The quantum system is initialized to an equal superposition, and the expectation value of the cost of Hamiltonian is measured. With classical methods, the parameters in cost and mixer can be optimized (cf. training in machine learning) so that we have a high probability of measuring the minimum eigenvalue and eigenstate of the cost Hamiltonian.

For a given cost Hamiltonian $H$ with $m$ terms, the parametrized cost unitary is defined as
\begin{equation*}
    U(\gamma) = e^{-i\gamma H} = \prod_{j = 1}^{m}e^{-i\gamma H_j},
\end{equation*}
where $H_j$ is the $j$th term. Theoretically, only a single parameter $\gamma$ suffices for each layer $p$. In practice, we noticed that even with large values of $p$, we were not able to find the correct parameters probably because the optimization problem became hard. Thus, we modified the algorithm so that we decreased the number of layers to one and increased the number of parameters using the following cost-unitary
\begin{equation*}
    U(\gamma_1, \ldots, \gamma_m) = \prod_{j = 1}^{m}e^{-i\gamma_j H_j}.
\end{equation*}
Instead of having a single parameter $\gamma$, we use $\gamma_j$ for every $ j = 1, \ldots, m$. This small modification seemed to make the optimization task easier in practice. Otherwise, we used the same mixer and measured the same expectation value as in the original QAOA algorithm.

Additionally, small HUBOs can be solved using D-Wave's Exact Poly Solver function, which simply enumerates all the possible solutions. The approach becomes infeasible with around 20 variables.
